Plane Wave Discontinuous Galerkin methods for the Helmholtz equation and Maxwell equations in Anisotropic Media

In this paper we are concerned with plane wave discontinuous Galerkin (PWDG) methods for Helmholtz equation and time-harmonic Maxwell equations in three-dimensional anisotropic media, for which the coefficients of the equations are matrices instead of numbers. We first define novel plane wave basis functions based on rigorous choices of scaling transformations and coordinate transformations. Then we derive the error estimates of the resulting approximate solutions with respect to the condition number of the coefficient matrices, under a new assumption on the shape regularity of polyhedral meshes. Numerical results verify the validity of the theoretical results, and indicate that the approximate solutions generated by the proposed PWDG method possess high accuracy.

==> chapter/chap-Con.tex <==
\section{Conclusion}


In this paper we have introduced a plane wave discontinuous Galerkin
method for discretization of the three-dimensional anisotropic Helmholtz equation
and time-harmonic Maxwell equations with the general positive definite matrix coefficients,
and derived  the optimal error estimate with respect to the condition number of the coefficient matrix
of the resulting approximate solutions.
We reported some numerical results to verify the validity of theoretical results,
and illustrate that the approximations generated by the proposed PWDG method 
possess high accuracies.

%are more accurate than those generated by other existing plane wave methods.






\iffalse
\vskip0.2in

{\bf Acknowledgments}. The authors wish to thank the anonymous
referee for many insightful comments which led to great improvement
in the results and the presentation of the paper.
\fi

